Query Answering in Lattice-based Description Logic

Recently, the description logic LE-ALC was introduced for reasoning in the semantic environment of the enriched formal contexts, and a tableaux algorithm was developed for checking the consistency of ABoxes in this logic. In this paper, we study the ontology-mediated query answering in LE-ALC . In particular, we show that several different types of queries can be answered efficiently for LE-ALC knowledge bases with acyclic TBoxes using our tableaux algorithm directly or by extending it with some additional rules.

==> eptcsdata.tex <==
\providecommand{\firstpage}{21}
\providecommand{\publicationstatus}{Cynthia Kop and Helida Salles Santos (Eds); 19th Workshop on\\ Logical and Semantic Frameworks with Applications (LSFA'24)\\
EPTCS 421, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.421.2}{10.4204/EPTCS.421.2}}
\pdfoutput=1

